Planning Landmark Based Goal Recognition Revisited: Does Using Initial State Landmarks Make Sense?

Goal recognition is an important problem in many application domains (e.g., pervasive computing, intrusion detection, computer games, etc.). In many application scenarios, it is important that goal recognition algorithms can recognize goals of an observed agent as fast as possible. However, many early approaches in the area of Plan Recognition As Planning, require quite large amounts of computation time to calculate a solution. Mainly to address this issue, recently, Pereira et al. developed an approach that is based on planning landmarks and is much more computationally efficient than previous approaches. However, the approach, as proposed by Pereira et al., also uses trivial landmarks (i.e., facts that are part of the initial state and goal description are landmarks by definition). In this paper, we show that it does not provide any benefit to use landmarks that are part of the initial state in a planning landmark based goal recognition approach. The empirical results show that omitting initial state landmarks for goal recognition improves goal recognition performance.

==> figures/adjusted.tex <==
\begin{figure}[h!]
	\centering
		\subfloat{
			\begin{tikzpicture}
			\pgfplotsset{every x tick label/.append style={font=\tiny}}
			\pgfplotsset{every y tick label/.append style={font=\tiny}}
				\begin{axis}[
					width=0.3\linewidth,
					height=5cm,
					xlabel={\scriptsize{Part of observation sequence}},
					ylabel={\scriptsize{Accuracy}},
					xlabel near ticks,
					ylabel near ticks,
					xmin=1, xmax=10,
					ymin=0, ymax=1.1,
					xtick={0,1,2,3,4,5,6,7,8,9,10, 11},
					xticklabels={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 0.99},
					ytick={0.2,0.4,0.6,0.8,1},
					legend pos=north west,
					ymajorgrids=false,
					xmajorgrids=false,
					major grid style={line width=.1pt,draw=gray!50},
					x axis line style={draw=black!60},
					tick style={draw=black!60},
					legend columns=3,
					legend style={draw=none},
					legend entries={\footnotesize{EX},\footnotesize{EX-init},\footnotesize{RHW},\footnotesize{RHW-init}},
					legend to name={average_performance}
				]

				\addplot[
					color=cyan,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.3528571428571428)(2.0,0.4078571428571429)(3.0,0.4707142857142858)(4.0,0.5007142857142858)(5.0,0.5807142857142857)(6.0,0.6528571428571429)(7.0,0.735)(8.0,0.7999999999999999)(9.0,0.8549999999999999)(10.0,0.9314285714285714)};

				\addplot[
					color=red,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.31285714285714283)(2.0,0.33285714285714285)(3.0,0.3935714285714286)(4.0,0.4278571428571429)(5.0,0.5007142857142857)(6.0,0.5564285714285714)(7.0,0.6592857142857144)(8.0,0.7371428571428572)(9.0,0.8192857142857142)(10.0,0.9235714285714286)};

				\addplot[
					color=orange,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.40071428571428575)(2.0,0.44)(3.0,0.5085714285714287)(4.0,0.5671428571428571)(5.0,0.6392857142857142)(6.0,0.7092857142857143)(7.0,0.7664285714285715)(8.0,0.8035714285714286)(9.0,0.8771428571428572)(10.0,0.9314285714285714)};

				\addplot[
					color=black,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.3514285714285715)(2.0,0.38714285714285707)(3.0,0.46571428571428575)(4.0,0.5285714285714286)(5.0,0.5942857142857143)(6.0,0.6742857142857144)(7.0,0.7335714285714285)(8.0,0.7728571428571429)(9.0,0.8614285714285715)(10.0,0.9235714285714286)};

				\end{axis}
			\end{tikzpicture}
			}
			\newline
			\vspace{-0.2cm}
	\ref{average_performance}
	\caption{Mean accuracy of the EX, EX-init, RHW, and RHW-init approaches on the \emph{average} domain.}

	\label{fig:average_performance}
\end{figure}

==> figures/adjusted_long.tex <==
\begin{figure}[h!]
	\centering
		\subfloat{
			\begin{tikzpicture}
			\pgfplotsset{every x tick label/.append style={font=\tiny}}
			\pgfplotsset{every y tick label/.append style={font=\tiny}}
				\begin{axis}[
					width=1\linewidth,
					height=5cm,
					xlabel={\scriptsize{Part of observation sequence}},
					ylabel={\scriptsize{Accuracy}},
					xlabel near ticks,
					ylabel near ticks,
					xmin=1, xmax=10,
					ymin=0, ymax=1.1,
					xtick={0,1,2,3,4,5,6,7,8,9,10, 11},
					xticklabels={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 0.99},
					ytick={0.2,0.4,0.6,0.8,1},
					legend pos=north west,
					ymajorgrids=false,
					xmajorgrids=false,
					major grid style={line width=.1pt,draw=gray!50},
					x axis line style={draw=black!60},
					tick style={draw=black!60},
					legend columns=3,
					legend style={draw=none},
					legend entries={\footnotesize{EX},\footnotesize{EX-init},\footnotesize{RHW},\footnotesize{RHW-init}},
					legend to name={average_performance}
				]

				\addplot[
					color=cyan,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.25)(2.0,0.32642857142857146)(3.0,0.3992857142857143)(4.0,0.4457142857142858)(5.0,0.527142857142857)(6.0,0.5928571428571429)(7.0,0.6685714285714285)(8.0,0.7321428571428571)(9.0,0.812142857142857)(10.0,0.9)};

				\addplot[
					color=red,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.1542857142857143)(2.0,0.17785714285714288)(3.0,0.24571428571428575)(4.0,0.2657142857142857)(5.0,0.3442857142857143)(6.0,0.3985714285714286)(7.0,0.5035714285714286)(8.0,0.6228571428571429)(9.0,0.7514285714285716)(10.0,0.8928571428571429)};

				\addplot[
					color=orange,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.2521428571428571)(2.0,0.31857142857142856)(3.0,0.4035714285714285)(4.0,0.4557142857142858)(5.0,0.5514285714285714)(6.0,0.6207142857142858)(7.0,0.6950000000000001)(8.0,0.7571428571428571)(9.0,0.8457142857142858)(10.0,0.9)};

				\addplot[
					color=black,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.22071428571428572)(2.0,0.26071428571428573)(3.0,0.34714285714285714)(4.0,0.4028571428571429)(5.0,0.49142857142857144)(6.0,0.5721428571428572)(7.0,0.6449999999999999)(8.0,0.7071428571428572)(9.0,0.8192857142857143)(10.0,0.8935714285714286)};

				\end{axis}
			\end{tikzpicture}
			}
			\newline
			\vspace{-0.2cm}
	\ref{average_performance}
	\caption{Mean accuracy of the EX, EX-init, RHW, and RHW-init approaches on the \emph{average} domain.}

	\label{fig:average_performance}
\end{figure}

==> figures/adjusted_short.tex <==
\begin{figure}[h!]
	\centering
		\subfloat{
			\begin{tikzpicture}
			\pgfplotsset{every x tick label/.append style={font=\tiny}}
			\pgfplotsset{every y tick label/.append style={font=\tiny}}
				\begin{axis}[
					width=1\linewidth,
					height=5cm,
					xlabel={\scriptsize{Part of observation sequence}},
					ylabel={\scriptsize{Accuracy}},
					xlabel near ticks,
					ylabel near ticks,
					xmin=1, xmax=10,
					ymin=0, ymax=1.1,
					xtick={0,1,2,3,4,5,6,7,8,9,10, 11},
					xticklabels={0.0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 0.99},
					ytick={0.2,0.4,0.6,0.8,1},
					legend pos=north west,
					ymajorgrids=false,
					xmajorgrids=false,
					major grid style={line width=.1pt,draw=gray!50},
					x axis line style={draw=black!60},
					tick style={draw=black!60},
					legend columns=3,
					legend style={draw=none},
					legend entries={\footnotesize{EX},\footnotesize{EX-init},\footnotesize{RHW},\footnotesize{RHW-init}},
					legend to name={average_performance}
				]

				\addplot[
					color=cyan,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.37785714285714284)(2.0,0.44071428571428567)(3.0,0.495)(4.0,0.5307142857142857)(5.0,0.6192857142857143)(6.0,0.6742857142857142)(7.0,0.7328571428571429)(8.0,0.8064285714285714)(9.0,0.8685714285714287)(10.0,0.9357142857142858)};

				\addplot[
					color=red,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.35500000000000004)(2.0,0.3885714285714285)(3.0,0.4457142857142857)(4.0,0.4714285714285714)(5.0,0.5428571428571429)(6.0,0.6178571428571428)(7.0,0.6900000000000002)(8.0,0.7692857142857142)(9.0,0.8442857142857144)(10.0,0.9292857142857142)};

				\addplot[
					color=orange,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.4585714285714286)(2.0,0.485)(3.0,0.5442857142857143)(4.0,0.5828571428571429)(5.0,0.6807142857142857)(6.0,0.7335714285714287)(7.0,0.7764285714285715)(8.0,0.8192857142857142)(9.0,0.8857142857142859)(10.0,0.9357142857142858)};

				\addplot[
					color=black,
						mark=none,
						dashed,
						]
						coordinates { (1.0,0.40285714285714286)(2.0,0.44571428571428573)(3.0,0.5135714285714286)(4.0,0.5592857142857144)(5.0,0.6421428571428572)(6.0,0.7114285714285715)(7.0,0.7585714285714287)(8.0,0.7964285714285716)(9.0,0.8842857142857145)(10.0,0.9292857142857142)};

				\end{axis}
			\end{tikzpicture}
			}
			\newline
			\vspace{-0.2cm}
	\ref{average_performance}
	\caption{Mean accuracy of the EX, EX-init, RHW, and RHW-init approaches on the \emph{average} domain.}

	\label{fig:average_performance}
\end{figure}

==> tables/adjusted.tex <==
\begin{table}
\caption{Comparison of evaluation results among different approaches (EX, EX-init, RHW, RHW-init, HM, HM-init) when applied to different benchmark domains. The accuracy is reported for different fractions $\lambda$ of the observation sequences that were used for recognition. Column \textbf{S} reports the average spread (size of the set of goals that are recognized as the true goal) for each domain.}

\label{tab:evaluationTable}
\resizebox*{0.5\columnwidth}{!}{
\begin{tabular}{ll|llllllllll|l}
\multicolumn{1}{c}{}		 & \multicolumn{1}{c|}{}		 & \multicolumn{10}{c|}{\textbf{Accuracy (for different $\lambda$)}}		 & \textbf{S} \\
			 & 			 & .1 		 & .2 		 & .3 		 & .4 		 & .5 		 & .6 		 & .7 		 & .8 		 & .9 		 & 1 		 & \\ \hline 
\multirow{6}{*}{\rotatebox[origin=c]{90}{blocks-world}}
 & A & \textbf{0.21} & \textbf{0.24} & \textbf{0.26} & .27 & .36 & .39 & \textbf{0.47} & \textbf{0.57} & \textbf{0.77} & \textbf{0.81} & 1.3\\
 & B & .17 & .17 & .21 & .22 & .32 & .34 & \textbf{0.47} & \textbf{0.57} & \textbf{0.77} & \textbf{0.81} & 1.3\\
 & C & .2 & .23 & \textbf{0.26} & \textbf{0.28} & \textbf{0.41} & \textbf{0.41} & \textbf{0.47} & \textbf{0.57} & .76 & \textbf{0.81} & 1.3\\
 & D & .2 & .22 & .23 & .27 & .35 & .37 & \textbf{0.47} & \textbf{0.57} & .75 & \textbf{0.81} & 1.2\\
 & E & . & .3 & .7 & .15 & .22 & .26 & .34 & .4 & .64 & .69 & 1.1\\
 & F & .5 & .1 & .13 & .13 & .19 & .24 & .28 & .35 & .61 & .66 & 1.1\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{depots}}
 & A & .21 & .29 & .28 & .32 & .37 & .39 & \textbf{0.63} & .67 & .76 & \textbf{0.93} & 1.4\\
 & B & .14 & .17 & .17 & .21 & .21 & .23 & .48 & .55 & .73 & \textbf{0.93} & 1.4\\
 & C & \textbf{0.23} & \textbf{0.33} & \textbf{0.29} & \textbf{0.45} & \textbf{0.42} & \textbf{0.55} & .62 & \textbf{0.82} & \textbf{0.89} & \textbf{0.93} & 1.3\\
 & D & .14 & .19 & .23 & .29 & .3 & .4 & .57 & .63 & .79 & \textbf{0.93} & 1.1\\
 & E & .9 & .5 & .5 & .5 & .9 & .18 & .36 & .39 & .57 & .68 & 1.3\\
 & F & .13 & .5 & .5 & .13 & .13 & .21 & .36 & .39 & .54 & .68 & 1.2\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{driverlog}}
 & A & .15 & .14 & .26 & .26 & .41 & .58 & .68 & .81 & \textbf{0.84} & \textbf{0.85} & 2.5\\
 & B & .16 & .15 & .19 & .19 & .24 & .35 & .39 & .55 & .64 & .74 & 1.3\\
 & C & \textbf{0.25} & \textbf{0.21} & \textbf{0.4} & \textbf{0.46} & \textbf{0.61} & \textbf{0.7} & \textbf{0.75} & \textbf{0.84} & \textbf{0.84} & \textbf{0.85} & 1.5\\
 & D & .15 & .15 & .24 & .21 & .36 & .48 & .49 & .65 & .69 & .74 & 1.4\\
 & E & .14 & .14 & .18 & .21 & .36 & .36 & .39 & .5 & .71 & .84 & 1.0\\
 & F & .4 & .4 & .7 & .11 & .29 & .32 & .32 & .46 & .61 & .77 & 1.1\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{dwr}}
 & A & .36 & .3 & \textbf{0.38} & .43 & .36 & \textbf{0.5} & \textbf{0.61} & .59 & .61 & \textbf{0.86} & 1.1\\
 & B & .39 & \textbf{0.32} & .32 & .36 & \textbf{0.39} & .39 & .46 & .5 & .61 & \textbf{0.86} & 1.0\\
 & C & \textbf{0.43} & .3 & .3 & \textbf{0.45} & \textbf{0.39} & \textbf{0.5} & .57 & \textbf{0.61} & \textbf{0.64} & \textbf{0.86} & 1.1\\
 & D & .36 & .27 & .32 & .32 & .32 & .46 & .57 & .54 & \textbf{0.64} & \textbf{0.86} & 1.1\\
 & E & .11 & .11 & .11 & .25 & .32 & .32 & .38 & .32 & .43 & .57 & 1.0\\
 & F & .14 & .21 & .21 & .25 & .32 & .36 & .39 & .32 & .43 & .57 & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{easy-ipc-grid}}
 & A & .17 & \textbf{0.25} & .32 & .35 & .38 & .41 & .44 & .57 & .77 & \textbf{1.0} & 1.8\\
 & B & .9 & .9 & .14 & .15 & .26 & .32 & .42 & .49 & .68 & \textbf{1.0} & 1.7\\
 & C & \textbf{0.23} & .2 & \textbf{0.35} & \textbf{0.4} & .4 & .46 & .54 & .55 & .7 & \textbf{1.0} & 1.2\\
 & D & .19 & .18 & .3 & .39 & \textbf{0.43} & \textbf{0.51} & \textbf{0.56} & .55 & .74 & \textbf{1.0} & 1.1\\
 & E & .17 & .19 & .24 & .33 & .41 & .44 & .53 & \textbf{0.61} & \textbf{0.78} & .95 & 1.6\\
 & F & .16 & .18 & .24 & .29 & .4 & .43 & .53 & \textbf{0.61} & \textbf{0.78} & .95 & 1.7\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{ferry}}
 & A & \textbf{0.53} & \textbf{0.75} & \textbf{0.75} & .77 & \textbf{0.84} & \textbf{0.88} & \textbf{0.96} & \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & 1.1\\
 & B & .35 & .45 & .45 & .55 & .71 & .71 & .82 & .89 & \textbf{0.95} & \textbf{0.96} & 1.0\\
 & C & \textbf{0.53} & \textbf{0.75} & \textbf{0.75} & .77 & \textbf{0.84} & \textbf{0.88} & \textbf{0.96} & \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & 1.1\\
 & D & .46 & .59 & .71 & \textbf{0.79} & .79 & .82 & .93 & \textbf{0.96} & \textbf{0.95} & \textbf{0.96} & 1.0\\
 & E & .29 & .57 & .64 & .68 & .82 & .86 & .89 & .93 & .93 & \textbf{0.96} & 1.0\\
 & F & .39 & .57 & .61 & .68 & .75 & .82 & .89 & .86 & .93 & \textbf{0.96} & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{intrusion-detection}}
 & A & .33 & .37 & .65 & \textbf{0.69} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
 & B & .33 & .37 & .65 & \textbf{0.69} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
 & C & .33 & .37 & .65 & \textbf{0.69} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
 & D & .33 & .37 & .65 & \textbf{0.69} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
 & E & \textbf{0.54} & \textbf{0.56} & \textbf{0.69} & \textbf{0.69} & .71 & .94 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
 & F & \textbf{0.54} & \textbf{0.56} & \textbf{0.69} & \textbf{0.69} & .71 & .94 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{logistics}}
 & A & .36 & \textbf{0.55} & \textbf{0.65} & \textbf{0.62} & \textbf{0.65} & \textbf{0.72} & \textbf{0.81} & \textbf{0.81} & \textbf{0.97} & \textbf{0.99} & 1.5\\
 & B & .21 & .31 & .49 & .55 & .56 & .62 & .78 & \textbf{0.81} & .94 & \textbf{0.99} & 1.1\\
 & C & \textbf{0.38} & .45 & .6 & .59 & .59 & .69 & .78 & .78 & \textbf{0.97} & \textbf{0.99} & 1.1\\
 & D & .28 & .4 & .56 & .58 & .58 & .68 & .78 & .78 & \textbf{0.97} & \textbf{0.99} & 1.1\\
 & E & .14 & .28 & .44 & .49 & .6 & .66 & .71 & \textbf{0.81} & .87 & .93 & 1.0\\
 & F & .19 & .27 & .45 & .49 & .6 & .61 & .71 & .8 & .86 & .91 & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{miconic}}
 & A & \textbf{0.71} & \textbf{0.75} & \textbf{0.82} & \textbf{0.86} & \textbf{0.82} & \textbf{0.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
 & B & .63 & .64 & .79 & .84 & \textbf{0.82} & \textbf{0.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
 & C & \textbf{0.71} & \textbf{0.75} & \textbf{0.82} & \textbf{0.86} & \textbf{0.82} & \textbf{0.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
 & D & .63 & .64 & .79 & .84 & \textbf{0.82} & \textbf{0.96} & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
 & E & \textbf{0.71} & .71 & .75 & .79 & \textbf{0.82} & .86 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
 & F & .64 & .66 & .71 & .71 & \textbf{0.82} & .86 & \textbf{1.0} & \textbf{1.0} & \textbf{1.0} & \textbf{0.98} & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{rovers}}
 & A & .3 & .38 & .39 & .45 & .57 & .59 & .79 & \textbf{0.86} & \textbf{0.86} & \textbf{0.86} & 1.7\\
 & B & .21 & .25 & .29 & .36 & .48 & .55 & .79 & .84 & \textbf{0.86} & \textbf{0.86} & 0.9\\
 & C & \textbf{0.46} & \textbf{0.6} & \textbf{0.68} & \textbf{0.71} & \textbf{0.79} & .8 & \textbf{0.86} & \textbf{0.86} & \textbf{0.86} & \textbf{0.86} & 0.9\\
 & D & .34 & .5 & .55 & \textbf{0.71} & .73 & \textbf{0.82} & .84 & \textbf{0.86} & \textbf{0.86} & \textbf{0.86} & 0.9\\
 & E & .21 & .27 & .3 & .36 & .57 & .57 & .75 & .79 & \textbf{0.86} & \textbf{0.86} & 0.9\\
 & F & .24 & .32 & .35 & .37 & .54 & .54 & .75 & .75 & \textbf{0.86} & \textbf{0.86} & 1.0\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{satellite}}
 & A & .25 & .3 & \textbf{0.4} & .4 & .55 & .69 & .76 & \textbf{0.93} & \textbf{0.96} & \textbf{0.96} & 2.5\\
 & B & .25 & .29 & .32 & .3 & .3 & .45 & .63 & .77 & .92 & \textbf{0.96} & 1.1\\
 & C & \textbf{0.34} & \textbf{0.34} & .37 & .44 & \textbf{0.58} & \textbf{0.71} & \textbf{0.84} & \textbf{0.93} & \textbf{0.96} & \textbf{0.96} & 1.2\\
 & D & .2 & .26 & .38 & \textbf{0.45} & .55 & \textbf{0.71} & .8 & \textbf{0.93} & \textbf{0.96} & \textbf{0.96} & 1.2\\
 & E & .17 & .17 & .24 & .3 & .37 & .54 & .72 & \textbf{0.93} & \textbf{0.96} & \textbf{0.96} & 1.4\\
 & F & .14 & .14 & .21 & .21 & .29 & .46 & .71 & \textbf{0.93} & \textbf{0.96} & \textbf{0.96} & 1.1\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{sokoban}}
 & A & .17 & .15 & .18 & .27 & .38 & \textbf{0.44} & .44 & \textbf{0.55} & .57 & .91 & 2.5\\
 & B & .2 & .2 & \textbf{0.24} & .28 & .36 & .41 & .45 & .53 & .46 & .91 & 2.2\\
 & C & .21 & .17 & .16 & .23 & \textbf{0.41} & .41 & \textbf{0.48} & .44 & \textbf{0.8} & .91 & 1.2\\
 & D & \textbf{0.24} & \textbf{0.24} & .17 & \textbf{0.29} & .39 & .35 & .42 & .46 & \textbf{0.8} & .91 & 1.2\\
 & E & .15 & .15 & .21 & .23 & .23 & .27 & .32 & .32 & .39 & .82 & 1.7\\
 & F & .17 & .17 & .23 & .24 & .36 & .35 & \textbf{0.48} & .49 & .48 & \textbf{0.95} & 1.6\\
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{zeno-travel}}
 & A & .22 & .24 & .25 & .32 & .44 & .59 & .7 & .88 & \textbf{0.91} & \textbf{0.93} & 2.9\\
 & B & .25 & .25 & .25 & .29 & .36 & .46 & .54 & .82 & \textbf{0.91} & \textbf{0.93} & 1.0\\
 & C & .34 & \textbf{0.46} & \textbf{0.49} & \textbf{0.61} & .69 & .86 & \textbf{0.86} & \textbf{0.89} & \textbf{0.91} & \textbf{0.93} & 1.2\\
 & D & \textbf{0.4} & .41 & .39 & .57 & \textbf{0.7} & \textbf{0.88} & .84 & \textbf{0.89} & \textbf{0.91} & \textbf{0.93} & 1.1\\
 & E & .4 & .4 & .7 & .18 & .23 & .33 & .44 & .73 & .86 & .89 & 1.2\\
 & F & .14 & .14 & .14 & .21 & .23 & .27 & .36 & .71 & .84 & .91 & 1.1\\
\hline
\end{tabular}
}
\end{table}
